Super-NaturalInstructions: Generalization via Declarative Instructions on 1600+ NLP Tasks

How well can NLP models generalize to a variety of unseen tasks when provided with task instructions? To address this question, we first introduce Super-NaturalInstructions, a benchmark of 1,616 diverse NLP tasks and their expert-written instructions. Our collection covers 76 distinct task types, including but not limited to classification, extraction, infilling, sequence tagging, text rewriting, and text composition. This large and diverse collection of tasks enables rigorous benchmarking of cross-task generalization under instructions -- training models to follow instructions on a subset of tasks and evaluating them on the remaining unseen ones. Furthermore, we build Tk-Instruct, a transformer model trained to follow a variety of in-context instructions (plain language task definitions or k-shot examples). Our experiments show that Tk-Instruct outperforms existing instruction-following models such as InstructGPT by over 9% on our benchmark despite being an order of magnitude smaller. We further analyze generalization as a function of various scaling parameters, such as the number of observed tasks, the number of instances per task, and model sizes. We hope our dataset and model facilitate future progress towards more general-purpose NLP models.

==> old_intro.tex <==
\begin{abstract}
How well can
% How can we measure if 
NLP models generalize to a \emph{variety} of unseen tasks when provided with the task instructions?
% their language instructions? 
%  Toward this goal, 
%  To measure ??, 
%  To facilitate progress in this goal, 
To address this question, 
% To address this question and facilitate future research towards general-purpose NLP models, 
 we introduce \name, a benchmark of 1,616 diverse NLP tasks and their expert-written instructions.
 Our collection covers 76 distinct task types, 
%  such as tagging, infilling, and rewriting. 
 including but not limited to classification, extraction, infilling, sequence tagging, text rewriting, and text composition.
 These tasks and their instructions are contributed by NLP practitioners and are passed through an iterative peer review process to ensure quality. 
% This benchmark enables large-scale evaluation of cross-task generalization of the models 
% With this large and diverse collection of tasks, we are able to rigorously benchmark cross-task generalization of models---training on a subset of tasks and evaluating on the remaining unseen ones.
This large and diverse collection of tasks enables rigorous benchmarking of cross-task generalization under instructions---training models to follow instructions on a subset of tasks and evaluating them on the remaining unseen ones.
\\
Specifically, 
% Using this data, 
we build  T\modelName{}, an encoder-decoder \underline{T}ransformer that is trained to follow a variety of in-context \underline{instructions} (plain language task definitions or \underline{$k$}-shot examples). 
Our experiments show this model outperforms existing 
instruction-following models such as InstructGPT by over 9\% on our benchmark despite of being orders of magnitude smaller. 
We further analyze generalization as a function of various scaling parameters, such as the number of observed tasks, the number of instances per task, and model sizes.
% We quantify generalization as a function of various scaling parameters, such as the number of observed tasks, the number of instances per task, and model sizes.
% Based on the insights,
% % Consequently, 
% we introduce T\modelName{}, an encoder-decoder \underline{T}ransformer that is trained to follow a variety of in-context \underline{instructions} (plain language task definitions or \underline{$k$}-shot examples), and outperforms existing 
% % larger models 
% instruction-following models 
% % that have orders of magnitude more parameters 
% such as InstructGPT by more than 8\% \todo{need update} despite of being orders of magnitude smaller.
% on our benchmark. 
We hope this benchmark facilitates future progress towards more general-purpose 
% language understanding models.
NLP models.\footnote{
The dataset and models
% , and evaluation scripts 
will be public upon publication. 
% are available at \textit{Anonymous URL}.\label{footnote:release} 
% The dataset, models, evaluation scripts, and leaderboard can be found at
% \url{https://instructions.apps.allenai.org}. 
\label{footnote:1}
% \todo{anonymize all footnotes}
}

\begin{comment}
% Humans (e.g., crowdworkers) have a remarkable ability in solving different tasks, by simply reading textual \emph{instructions} that define them and looking at a few examples. 
% Despite the success of the conventional supervised learning on individual datasets, such models often struggle with generalization across tasks (e.g., a question-answering system cannot solve  classification tasks).
%  A long-standing challenge in AI is to build a model that learns a new task by understanding the human-readable \emph{instructions} that define it.
%  The recent literature has shown the propensity of pre-trained neural language models in 
%  The recent literature has shown promising trends in generalization of pre-trained neural language models  to unseen tasks when fine-tuned to follow task instructions. 
How can we measure the generalization of models to a \emph{variety} of unseen tasks when provided with their language instructions? 
 To facilitate progress in this goal, we introduce \name,  a collection of 1,600+  diverse 
 NLP tasks 
%  language tasks 
%  (i.e., mapping an input text to an output text)\swaroop{remove "(mapping an input text to an output text)"}\daniel{hmm, without this is it clear with "task" means?}, 
 and their expert written instructions. 
%  Besides its size, this benchmark contains a variety of 
More importantly, it covers 70+ distinct task types, such as tagging, in-filling, and rewriting. 
%  The instructions are obtained from crowdsourcing instructions used to create  existing NLP datasets and  mapped to a unified schema. 
 These tasks are collected with contributions of NLP practitioners in the community and through an iterative peer review process to ensure their quality. 
%  quality is improved through several rounds of  
%  d via a large-scale community effort and 
%  their quality is improved with several rounds of peer reviews. 
%  Using this meta-dataset, 
This benchmark enables large-scale evaluation of cross-task generalization of the models---training on a subset of tasks and evaluating the remaining unseen ones.
For instance, we are able to rigorously 
% conduct extensive experiments to 
quantify generalization as a function of various scaling parameters, such as 
% the number of observed tasks, 
% or their categories \yizhong{remove categories?}, 
% model sizes, and the number of examples 
the number of observed tasks, the number of instances, and model sizes.
% As a by-product of these experiments,
Based on these insights,
% we introduce T\modelName{}\swaroop{what does TK stand for? May be we can have a name which is easy to remember e.g. "Instruction-follower" or "Instruct-me"} models that are trained to 
% a generative model  that 
% \hanna{what does this mean? accept a variety? that are trained to generate the task output .....} accepts a variety of in-context instructions (plain language task definitions or $k$-shot examples) that outperforms other relevant and larger models on our benchmark.
we introduce T\modelName{}, an encoder-decoder \underline{T}ransformer that is trained to follow a variety of in-context \underline{instructions} (plain language task definitions or \underline{$k$}-shot examples) which outperforms existing larger models on our benchmark.
% In particular, \todo{ONE SPECIFIC OBSERVATION}
% In particular, while models consistently learn to get better at following language instructions, 
%  Our results indicate that models \emph{benefit from instructions} when evaluated in terms of generalization to unseen tasks (19\% better for models utilizing instructions). 
%  These models, however, are far behind  an estimated performance upper-bound, indicating significant room for more progress in this direction.
% \todo{say something about the empirical findings.}
We hope this benchmark facilitates future progress toward more general-purpose language understanding models.\footnote{
% Dataset is available at 
The dataset, models, evaluation scripts and a leaderboard can be found 
% \yizhong{will be released?} 
at 
\url{https://instructions.apps.allenai.org}
% \href{https://github.com/allenai/natural-instructions}{\nolinkurl{https://github.com/allenai/natural-instructions}}
\label{footnote:1}
}
\end{comment}

% \blfootnote{$\diamondsuit$ Co-first authors $\clubsuit$ Co-second authors}

\end{abstract}

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.63,trim=9.2cm 7cm 9.2cm 4.2cm]{figures/Example-v2.pdf}
%     \caption{An example of a task in \nameShort. 
%  %   \yizhong{I like this new figure. Probably we can also put definition in a box? And the other info as a Meta Info box? }}
%   %  \yeganeh{Yeah, I'll try that}
%   \todo{Working on merging this with figure \ref{fig:schema}}
%   }
%     \label{fig:example}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth,trim=0cm 0.2cm 0cm 1cm]{figures/fig1-v8.pdf}
    % \includegraphics[scale=0.3,trim=5.4cm 8.5cm 3cm 2.5cm,clip=true]{figures/fig1-v7.pdf}
    \caption{An example task from \nameShort{} adopted from \citet{chawla2021casino}. 
    % of a negotiation strategy detection task (from CaSiNo; \citealp{chawla2021casino}) in \nameShort. 
    % Note that it follows the instruction schema detailed in (\S\ref{schema}). 
    A successful model is expected to use the provided instructions (including task definition and demonstration examples) to output responses to a pool of evaluation instances. 
    % The goal for the model is to generate the expected output from the given input by leveraging the task instructions that describe the task.
 %   \yizhong{I like this new figure. Probably we can also put definition in a box? And the other info as a Meta Info box? }}
  %  \yeganeh{Yeah, I'll try that}
%   \todo{Working on merging this with figure \ref{fig:schema}}
  }
    \label{fig:example}
\end{figure}

\section{Introduction}
Building general-purpose models that can follow 
% a broad variety of 
language instructions to solve tasks has been a long aspired goal of AI~\cite{winograd1972understanding}. 
Backed by large pretrained language models~\cite{raffel2020exploring,brown2020language}, the recent literature has shown evidence on models' ability to 
% tackled this goal by benchmarking models' ability to 
generalize to \emph{unseen} tasks via instructions~\cite{mishra2022cross, jang2022bc,ouyang2022training}.  
% Building models that can follow language instructions and generalize to \emph{unseen} tasks has received increased attention in recent literature~\cite{mishra2022cross, wei2022finetuned,sanh2022multitask, ouyang2022training}. 
% All these efforts are enabled with datasets of tasks and their instructions that 
% For instance, \citet{mishra2022cross} showed linearly improving cross-task generalization as a function of observed tasks, however, 
% Despite such promising observations, there is little understood about the limitations of such approaches~\cite{webson2022do}. 
% Despite such promising observations, there is little understood about the limitations of such approaches~\cite{webson2022do}. 
% \daniel{need better transition here; need to highlight limitations with the earlier datasets and motivate the necessitate the construction of a more broad-reaching benchmark. 
% one transition can use the the analysis of \citet{webson2022do} to highlight weaknesses in these models. 
% }
Meanwhile, the community's understanding in regards to the limitations of these approaches is evolving~\cite{webson2022do,min2022rethinking}. 
A bottleneck for better characterizing the success and limitations of this line of work is the availability of benchmarks with a broad \emph{variety} of tasks and their instructions (see Table~\ref{tab:dataset_comparison}).




\input{tables/dataset_comparison}


\begin{figure*}
\centering
\begin{tabular}{cccc}
\multicolumn{2}{c}{
\multirow{2}{*}{
    \begin{minipage}[b][][t]{0.4\textwidth}\vspace{0pt}
	\begin{subfigure}[b][1\width]{1\textwidth}
	   \includegraphics[trim= 2cm 0.3cm 0cm 3cm, width=1.14\textwidth]{figures/NLI2.pdf}
	   \captionsetup{font=scriptsize}\caption{\nameShort{} (this work) \label{figure:visualization-nli2}}
	\end{subfigure}
	\end{minipage}
}} & \begin{subfigure}[c][1\width]{
	   0.22\textwidth}
	   \includegraphics[width=1\textwidth]{figures/NLI1.pdf}
	   \captionsetup{font=scriptsize}\caption{\naturalinsShort \label{figure:visualization-nli1}}
	\end{subfigure} &
	\begin{subfigure}[c][1\width]{
	   0.22\textwidth}
	   \includegraphics[width=1\textwidth]{figures/Promptsource.pdf}
	   \captionsetup{font=tiny}\caption{\promptsource~(T0 subset) \label{figure:visualization-ps}}
	\end{subfigure}	
	\\[2.1cm]
\multicolumn{2}{c}{} &
    \begin{subfigure}[c][1\width]{
	   0.22\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{figures/flan.pdf}
	   \captionsetup{font=scriptsize}\caption{\flan \label{figure:visualization-flan}}
	\end{subfigure} &
	\begin{subfigure}[c][1\width]{
	   0.22\textwidth}
	   \centering
	   \includegraphics[width=1\textwidth]{figures/gpt3.pdf}
	   \captionsetup{font=scriptsize}\caption{\gptthree \label{figure:visualization-gpt}}
	\end{subfigure} \\
	\end{tabular}
	\vspace{5pt}
    \caption{
    Compared to other datasets, \nameShort{} covers a more diverse range of task types. InstructGPT reports a very coarse categorization of their task types. Bubble size represents the number of tasks of each type in log scale.}    
    \label{fig:visualizations}
\end{figure*}


We introduce \name{} (\nameShort{} for short), a large benchmark of 1,616 NLP tasks and their language instructions.
This meta-dataset (i.e., dataset of datasets~\cite{triantafillou2019meta}) brings in a
variety of tasks---76 task types 
% \todo{x} reasoning types, \cite{x} domains, 
spanning 55 different languages.
Each task is paired up with an instruction that consists of the task definition for mapping an input text to a task output and several examples for demonstrating the desired or undesired output (see Fig.\ref{fig:example} as an example task).
% Each task consists of a task instruction in natural language that provides the task definition for mapping an input text to a task output followed by a few task instances (see Fig.\ref{fig:example} as an example task).
% For instance, Fig.\ref{fig:example} shows the instructions of a negotiation strategy detection task. 
The data was collected by contributions of various NLP practitioners, in response to our public call for contributions, and it is mostly based on existing NLP datasets. 
These contributions are consolidated after several rounds of peer-review and crowdsourced feedback to ensure the quality of the collected instructions. Table~\ref{tab:dataset_comparison} and Figure~\ref{fig:visualizations} highlight  properties of \nameShort{} compared to  relevant benchmarks, emphasizing on the diversity of tasks and instruction types in our benchmark.
% \daniel{It might helpful to refer to an example, somewhere around here; so far, it is not clear what is it that we're talking about. }
% This is complemented with crowdworker-based estimation of data quality which indicates the quality of the collected task instructions.
% We do human quality verification where we observe that humans do quite well. 
% \daniel{we may need to clarify why we call these "**in-context** instructions". }

We hope \nameShort{} can facilitate research towards generalizable NLP models.
% \nameShort{}  facilitates research towards building generalizable NLP models that can follow instructions, where they will be evaluated by task instances. %  can 
% The goal is to evaluate if a model can 
%perform the task (evaluated by task instances) by following the provided in-context task instructions---an extension to the example-based in-context learning setup \cite{brown2020language}.
In particular, we showcase its application for studying generalization to unseen tasks in many languages, given their plain English instructions (\S\ref{sec:empirical}). 
Having this diverse and large-scale data enables us to carefully split our tasks into training and test sets, and systematically study how state-of-the-art methods perform on them. % Our empirical results indicate that, while existing prompt-based models (such as InstructGPT \cite{ouyang2022training}) demonstrate some ability to follow the instructions, they generally cannot easily transfer to our instruction schema. 
% For example, this enables scaling experiments on the size of supervision tasks, their instances and model sizes (\S\ref{subsec:scaling}). 

% Further analysis shows the important instruction elements (e.g., definition, demonstration examples), the benefit of including more training tasks, and the effect of model scale.
Furthermore, we build T\modelName{}, a generative model for transforming 
task input (sentences, paragraphs, etc.)
according to declarative in-context instructions (language definition or $k$-shot examples). 
% a flexible combination of $k$-shot examples and language instructions.
% This 3B \nascomment{-parameter ?} model that is trained on our data 
% % enable better instruction following. 
% % A 3B T5 model finetuned on our training tasks can 
% outperforms the 175B InstructGPT model~\cite{ouyang2022training} by 3.3\% and 7.9\% when evaluated on 119 English and 35 non-English evaluation tasks (\S\ref{subsec:main_results}). 
Our T\modelName{} is  built by training a T5 model~\cite{raffel2020exploring} on our data. Interestingly, a T5-11B model finetuned on our training tasks can 
outperform the 175B-parameter InstructGPT model~\cite{ouyang2022training} by 9.9 ROUGE-L points when evaluated on 119 unseen English tasks, and its multilingual variant mT\modelName{} outperforms InstructGPT by 13.3 points on 35 non-English tasks (\S\ref{subsec:main_results}).
% \daniel{need to refer to x-lingual experiments and emphasize the importance: To the best of our knowledge, this is the first study in cross-lingual cross-task generalization.}

Finally, we provide various analyses and estimate performance upper bounds, which suggests further room for improvement. \todo{include the analysis finding here.

}
% We hope that this data will facilitate further progress toward better instruction-following systems.


  
% Overall, while we believe that our instructions should provide enough information for solving the tasks, current tested methods still have a large gap behind supervised approach and human beings 
% Overall, while we believe that our instructions should provide enough information for solving tasks, current methods that follow the instructions to do unseen tasks still under-perform supervised approach and human beings by a large margin.
% \daniel{the purpose of the previous sentence is not quite clear; I think we should explicitly articulate something like: "leaves room for improvement", which can tie with motivating future research.}
%  - We can use it for cross-task generalization, as it has been used before: 
% Cross-task generalization -- \emph{generalization} to  \emph{unseen} tasks -- has recent 
%  \todo{
%  - Summarize our empirical findings for this setup: .... 
%  - End with other potential uses of the data. 
%  } \yizhong{added the summarization for empirical results.}
  % \yeganeh{Due to the similarity between this sentence and the last sentence of the abstract, maybe change to sth like: We hope this data will contribute to improving instructions-following systems in the future.}



==> old_text.tex <==
\begin{comment}
% (e.g., GPT3~\cite{brown2020language}).
% The recent developments  on  
% developments in building models for following 
% generalization to 
% \emph{unseen} 
% in-context instruction
% such as InstructGPT3~\cite{ouyang2022training} 
% have resulted  in models with spectacular  
% have been shown an impressive
% ability in following declarative instructions instructions~\cite{mishra2022cross,jang2022bc,ouyang2022training}. 
As impressive as models like InstructGPT3~\cite{ouyang2022training} are, 
% it not quite well-understood how much various factors contribute to their success:  
% it not quite well-understood how various design choices contribute to  their success: 
% it not quite well-understood their success to what extend is indebted to various design choices: 
% it not quite well-understood their quality to what extend is indebted to various design choices: 
the contribution of various design choices to their success 
(enormity of their models, their supervision data and so on)  is  opaque. 
In particular, the role of supervised data has remained understudied due to limited data released by major corporate entities behind major models. 
Addressing this question necessitates availability large-scale benchmarks of language instructions for a broad range of tasks.

% how much does the enormous model help? 
% for example, how much does the enormity of the models help? 
% how necessary is the enormity of the models? 
% is it the algorithm for incorporating their supervision? 
% how about the supervision algorithm? 
% orthe data used for supervising such models? 
% how about the underlying algorithm? 
% last but not least, 
% or, how crucial is large-scale supervision data? 
% In particular, the latter question has remained 
% The latter issue in particular  has remained 
% opaque and understudied because of 
% of the strict  data release of
% limited data released 
% meager data release by corporate entities behind major models, 
% and 
% relatively small scale of available benchmarks.
% This highlights the need for large-scale and diverse  dataset for measure various forms of generalizagtion. 
\end{comment}

==> tables/test_categories_and_examples.tex <==
\begin{comment}
\begin{table*}[ht]
\label{tab:test_categories_and_examples}
\centering
\tiny
\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{0.06\textwidth}|p{0.06\textwidth}|p{0.07\textwidth}|p{0.07\textwidth}|p{0.39\textwidth}|p{0.39\textwidth}|p{0.39\textwidth}|}
\hline
\multirow{2}{*}{Category} & \multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Example Task from the Category}                                                   \\ \cline{3-7} 
 &  & \multicolumn{1}{c|}{Task Name} & \multicolumn{1}{c|}{Source Dataset} & \multicolumn{1}{c|}{Definition} & \multicolumn{1}{c|}{Positive Example} & \multicolumn{1}{c|}{Negative Example} \\ 
 
 \hline
Textual   Entailment &
  Exact   Match &
  task1344 glue entailment classification &
  RTE &
  In   this task, you're given two sentences. Indicate if the first sentence clearly   entails the second sentence (i.e., one can conclude the 2nd sentence by   reading the 1st one). Indicate your answer with '1' if the first sentence   entails the second sentence, otherwise answer with '0'. &
  Input:   Sentence 1: No Weapons of Mass Destruction Found in Iraq Yet. Sentence   2:Weapons of Mass Destruction Found in Iraq. Output: 0 Explanation: In our   first statement we clearly say that Iraq does not have any weapon of mass   destruction but the second sentence says that weapon of mass destruction is   found in Iraq which is a contradiction. Hence output will be 0 for non   entailment. &
  Input:   Sentence 1: Valero Energy Corp., on Monday, said it found   "extensive" additional damage at its 250,000-barrel-per-day Port   Arthur refinery. Sentence 2: Valero Energy Corp. produces 250,000 barrels per   day. Output: 0 Explanation: The first statement mentions that there was   damage found in the 250,000 barrel-per-day Port Aurthur refinery. Which means   that they produce 250,000 barrels a day. Hence the output should have been 1   for entailment \\ \hline
Cause   Effect Classification &
  Exact   Match &
  task828 copa commonsense cause effect &
  COPA &
  In   this task your given two statements. You must judge whether the second   sentence is the cause or effect of the first one. Label the instances as   "cause" or "effect" based on your judgment. The sentences   are separated by a newline character. &
  Input:   The women met for coffee. They wanted to catch up with each other. Output:   cause Explanation: The women met for coffee because they wanted to catch up   with each other. &
  Input:   My body cast a shadow over the grass. The sun was rising. Output: effect   Explanation: The rising of the sun isn't an effect of casting a shadow over   the grass. \\ \hline
Coreference   Resolution &
  Exact   Match &
  task1391 winogrande easy answer generation &
  Winogrande &
  In   this task, you are given a question containing a blank (\_) and two options.   You should pick the best option to answer the question. Please answer with   "A" or "B". &
  Input:   Katrina gave Christine a stuffed animal for their birthday, but \_ already had   this one. (A) Katrina (B) Christine Output: B Explanation: Since the blank is   someone who received the gift and already had a stuffed animal, the answer   must be "Christine". &
  Input:   Ian got into position and punched Lawrence so hard that his mouthpiece flew   right out because \_ was a quick fighter. (A) Ian (B) Lawrence Output: C   Explanation: The issue is that the answer is not one of the options presented   in the question which are "A" and "B". Note that, a valid   answer must be one of the options. \\ \hline
Dialogue   Act Recognition &
  Exact   Match &
  task1394 meta woz task classification &
  Meta WOZ &
  In   this task, you are given four sentences: a bot task sentence, a bot role   sentence, a user task sentence and a user role sentence. Your job is to   classify given sentences into one of the 47 different domains. The domains   are: 'UPDATE\_CALENDAR', 'PRESENT\_IDEAS', 'MOVIE\_LISTINGS', 'AUTO\_SORT',   'GAME\_RULES', 'CONTACT\_MANAGER', 'BANK\_BOT', 'MUSIC\_SUGGESTER',   'CHECK\_STATUS', 'PET\_ADVICE', 'HOW\_TO\_BASIC', 'NAME\_SUGGESTER',   'QUOTE\_OF\_THE\_DAY\_BOT', 'GUINESS\_CHECK', 'INSURANCE', 'RESTAURANT\_PICKER',   'MAKE\_RESTAURANT\_RESERVATIONS', 'WEDDING\_PLANNER', 'SKI\_BOT', 'HOME\_BOT',   'PLAY\_TIMES', 'BUS\_SCHEDULE\_BOT', 'WHAT\_IS\_IT', 'PHONE\_PLAN\_BOT',   'DECIDER\_BOT', 'PHONE\_SETTINGS', 'TIME\_ZONE', 'LIBRARY\_REQUEST',   'UPDATE\_CONTACT', 'CATALOGUE\_BOT', 'PROMPT\_GENERATOR', 'SCAM\_LOOKUP',   'SPORTS\_INFO', 'POLICY\_BOT', 'CITY\_INFO', 'APARTMENT\_FINDER',   'EVENT\_RESERVE', 'SHOPPING', 'EDIT\_PLAYLIST', 'LOOK\_UP\_INFO', 'ORDER\_PIZZA',   'WEATHER\_CHECK', 'APPOINTMENT\_REMINDER', 'GEOGRAPHY', 'STORE\_DETAILS',   'AGREEMENT\_BOT', 'ALARM\_SET'. &
  Input:   Bot's task: Inform the user that the topping they are asking for is   unavailable Bot's role: You are a bot designed to help customers order pizza   User's task: Ask if a certain pizza topping is available User's role: You are   interacting with a pizza restaurant bot Output: ORDER\_PIZZA Explanation:   According to the descriptions of the four sentences, we know that the type of   task is ORDER\_PIZZA &
  Input:   Bot's task: Help the user with their pizza order Bot's role: You are a bot   designed to help customers order pizza User's task: Ask the bot for three   different pizzas User's role: You are interacting with a pizza restaurant bot   Output: UPDATE\_CALENDAR Explanation: According to the descriptions of the   tasks and roles, we know that the type of task is ORDER\_PIZZA, but the output   is UPDATE\_CALENDAR, so it is incorrect. \\ \hline
Answerability   Classification &
  Exact   Match &
  task1640 aqa1.0 answerable unanswerable question classification &
  Adversarial QA &
  Given   a paragraph from a wikipedia article about some topic, and a question related   to the topic, determine whether the question is answerable from the   paragraph. If the question is answerable, answer "True", otherwise,   answer "False". &
  Input:   Another approach to brain function is to examine the consequences of damage   to specific brain areas. Even though it is protected by the skull and   meninges, surrounded by cerebrospinal fluid, and isolated from the   bloodstream by the blood–brain barrier, the delicate nature of the brain   makes it vulnerable to numerous diseases and several types of damage. In   humans, the effects of strokes and other types of brain damage have been a   key source of information about brain function. Because there is no ability   to experimentally control the nature of the damage, however, this information   is often difficult to interpret. In animal studies, most commonly involving   rats, it is possible to use electrodes or locally injected chemicals to   produce precise patterns of damage and then examine the consequences for   behavior. Question: What is surrounded by cerebrospinal fluid? Output: True   Explanation: The paragraph comes from the wikipedia page on the brain. The   answer to the question is the brain which can be found in the paragraph. &
  Input:   NASCAR (headquartered in Daytona Beach) begins all three of its major auto   racing series in Florida at Daytona International Speedway in February,   featuring the Daytona 500, and ends all three Series in November at   Homestead-Miami Speedway. Daytona also has the Coke Zero 400 NASCAR race   weekend around Independence Day in July. The 24 Hours of Daytona is one of   the world's most prestigious endurance auto races. The Grand Prix of St.   Petersburg and Grand Prix of Miami have held IndyCar races as well. Question:   What is the starting time of NASCAR's big events? Output: False Explanation:   This paragraph comes from the wikipedia article on Florida. The answer to the   given question is February which can be found in the paragraph, however the   output is given as False. \\ \hline
Word   Analogy &
  Exact   Match &
  task1156 bard  analogical reasoning tools &
  BARD &
  Two   analogies that relate actions to the tools used to perform the action is   given in the form "A : B. C : ?". "A : B" relates action   A to tool B. Your task is to replace the question mark (?) with the   appropriate tool for the given action C, following the "A : B"   relation. &
  Input:   eat : fork. cook : ? Output: pan Explanation: The given analogy relates   actions to the tools used to perform them. A fork can be used to eat. To   cook, a pan can be used. &
  Input:   dig : shovel. wash : ? Output: sink Explanation: The given analogy relates   actions to the tools used to perform them. A knife can be used to cut. To   wash, a sink CANNOT be used. \\ \hline
Overlap   Extraction &
  ROUGE-L &
  task281 points of correspondence &
  Points of Correspondence &
  You   will be given three sentences. Read them, then identify a noun phrase   (person, place, or thing) or event that is shared between all three   sentences. As the output, write the span of the text corresponding to that   phrase in each sentence. &
  Input:   sentence 1: Four employees of the store have been arrested , but its manager   -- herself a woman -- was still at large Saturday , said Goa police   superintendent Kartik Kashyap . sentence 2: If convicted , they could spend   up to three years in jail , Kashyap said . sentence 3: The four store workers   arrested could spend 3 years each in prison if convicted . Output: sentence   1: Four employees of the store sentence 2: they sentence 3: The four store   workers Explanation: All three mentioned parts refer to the same entity, the   four eployees. "Of the store" in first sentence must be included,   since it is part of the same noun phrase describing the employees. &
  Input:   sentence 1: Stewart said that she and her husband , Joseph Naaman , booked   Felix on their Etihad Airways flight from the United Arab Emirates to New   York 's John F . Kennedy International Airport on April 1 . sentence 2: The   couple said they spent $ 1,200 to ship Felix on the 14-hour flight . sentence   3: Couple spends $ 1,200 to ship their cat , Felix , on a flight from the   United Arab Emirates . Output: sentence 1: she and her husband sentence 2:   couple sentence 3: Couple Explanation: Mentioning only "she and her   husband" in sentence 1 would be incorrect, because "Joseph   Naaman" is part of the same noun phrase. Similarly, mentioning only   "couple" in sentence 2 would be incorrect; you must mention   "the couple." \\ \hline
Keyword   Tagging &
  ROUGE-L &
  task036 qasc topic word to generate related fact &
  QASC &
  In   this task, you need to write a topic word from the given fact. The topic word   must have at least one word overlap with the given fact. The topic word often   involves adding a new word from a related concept. Things to avoid: -   Emphasis \& Caution: 1. In your topic word, use at least one word from the   given Fact. 2. Topic words with two or more words work best. &
  Input:   Fact: pesticides cause pollution. Output: pollution harms. Explanation: This   is a good topic word, because it contains one overlapping word   "pollution". &
  Input:   Fact: pesticides cause pollution. Output: computer harms. Explanation: This   is a bad topic word, because it has no overlapping word with the given fact. \\ \hline
Question   Rewriting &
  ROUGE-L &
  task1622 disfl qa text modication &
  Disfl QA &
  Convert   a disfluent question to a proper question. A disfluent question is a question   that has some interruptions in it while framing. A proper question is the   correct form of the question without any disfluency. &
  Input:   Why was uh where was the Rhine regulated with an upper canal? Output: Where   was the Rhine regulated with an upper canal? Explanation: The above disfluent   question is correctly converted to a proper question. The 'uh' and the 'why'   before the correction should be removed to make it fluent. &
  Input:   When did Maududi exert the least impact no where did he exert? Output: When   did Maududi exert the least impact? Explanation: The above disfluent question   is not correctly converted to a proper question since the original meaning in   the disfluent question is where did Maudidi exert the least impact but the   output asks when did Maudidi exert the least impact. \\ \hline
Title   Generation &
  ROUGE-L &
  task418 persent title generation &
  PRESENT &
  Given   a document, generate a short title of the document. The title should convey   the main idea/event/topic about which the document is being written. Note   that URLs in the text have been replaced with {[}Link{]}. &
  Input:   In a letter posted on the White House web site Tuesday John Brennan assistant   to President Barack Obama for homeland security and counterterrorism said   Schmidt will have regular access to the president and play a vital role in   the country's security. Schmidt's selection comes more than 10 months after   Obama declared cyber security a priority and ordered a broad administration   review. A senior White House official said Obama was personally involved in   the selection process and chose Schmidt because of his unique background and   skills. Schmidt will have regular and direct access to the president for   cyber security issues the official said. The official spoke on the condition   of anonymity to discuss the selection process. At the same time cyber experts   and potential job candidates have complained that the position lacks the   budgetary and policy-making authority needed to be successful. Schmidt will   report to the National Security Council and closely support the National   Economic Council on cyber issues. Schmidt's selection suggests that economic   and business interests in the White House held more sway in the selection   process. Schmidt president and CEO of the Information Security Forum a   nonprofit international consortium that conducts research in information   security has served as chief security officer for Microsoft and as cyber   security chief for online auction giant eBay. He was reportedly preferred by   Lawrence Summers director of the economic council. Output: White House picks   new cyber coordinator Explanation: The title is relevant to the main topic of   document, that is, the selection of Schmidt as the cybersecutiy chief. &
  Input:   LeBron James has had a strong response after a Fox News host said that   instead of criticizing President Donald Trump he should just "shut up   and dribble." This isn't the first time James has used his shoes to make   a statement. In December when the Cavs played in D.C. he wore black and white   sneakers that said "Equality." Output: Fox News host asked LeBron   to shut up Explanation: This is not the main topic of the document. The main   topic is about LeBron wearing shoes to make public statements which is   supported by the last sentence as well. \\ \hline
Data   to Text &
  ROUGE-L &
  task957 e2e nlg text generation generate &
  E2E &
  In   this task, we ask you convert a data table of restaurant descriptions into   fluent natural-sounding English sentences. The input is a string of key-value   pairs; the output should be a natural and grammatical English sentence   containing all the information from the input. &
  Input:   name{[}Aromi{]}, eatType{[}restaurant{]}, food{[}English{]}, area{[}city centre{]} Output:   Aromi is an English restaurant in the city centre. Explanation: The output   sentence faithfully converts the data in the input into a natural-sounding   sentence. &
  Input:   name{[}Blue Spice{]}, eatType{[}coffee shop{]}, priceRange{[}more than £30{]}, customer   rating{[}5 out of 5{]}, area{[}riverside{]}, familyFriendly{[}yes{]}, near{[}Avalon{]}   Output: Blue Spice is a Colombian coffee shop located by the riverside, near   Avalon in Boston. Its prices are over £30. Its customer ratings are 5 out of   5. Explanation: While the output contains most of the information from the   input, it hallucinates by adding ungrounded information such as   "Colombian" and "Boston". \\ \hline
Grammar   Error Correction &
  ROUGE-L &
  task1557 jfleg answer generation &
  JFLEG &
  In   this task, you will be shown an incorrect English sentence. You need to   generate a corrected form of the input sentence. &
  Input:   The car's wheel are loose. Output: The car's wheel is loose. Explanation: The   instance of are is replaced by the word is. This makes the sentence   grammatically correct. &
  Input:   This way is the way to go. Output: This way may be the way to go.   Explanation: The example does not correct the misuse of the word way.   Instead, it should shorten the sentence to: this is the way to go. \\ \hline

\end{tabular}%
}
\caption{12 Evaluation categories (\S\ref{subsec:setup}), their evaluation metrics (Exact Matching or ROUGE-L, \S\ref{subsec:metrics}), and representative tasks for each category.}
\end{table*}

\end{comment}

==> tables/transferring_results_across_encodings.tex <==
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Testing Encoding →\\ Training Encoding ↓\end{tabular} &
  task name &
  instruct &
  pos (1) &
  \begin{tabular}[c]{@{}c@{}}instruct \\ + pos (1)\end{tabular} &
  pos (2) &
  \begin{tabular}[c]{@{}c@{}}instruct \\ + pos (2)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}instruct \\ + pos (2) \\ + neg (2)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}instruct \\ + pos (2) \\ + neg (2) \\ + expl.\end{tabular} &
  pos (4) &
  \begin{tabular}[c]{@{}c@{}}instruct \\ + pos (4)\end{tabular} &
  Average \\ \hline
task name &
  \underline{ 21.22} &
  33.25 &
  16.77 &
  30.95 &
  22.97 &
  33.70 &
  33.87 &
  31.55 &
  25.98 &
  36.36 &
  33.95 \\ \hline
instruct &
  17.30 &
  \underline{ 44.96} &
  31.06 &
  43.78 &
  36.42 &
  46.41 &
  44.17 &
  44.27 &
  37.97 &
  45.99 &
  39.92 \\ \hline
pos (1) &
  10.87 &
  22.07 &
  \underline{ 43.90} &
  47.81 &
  46.58 &
  49.21 &
  46.16 &
  43.43 &
  46.61 &
  49.53 &
  43.13 \\ \hline
instruct + pos (1) &
  11.09 &
  42.24 &
  43.81 &
  \underline{ 52.38} &
  47.35 &
  53.25 &
  53.06 &
  51.80 &
  47.80 &
  53.65 &
  44.49 \\ \hline
pos (2) &
  12.74 &
  22.40 &
  47.07 &
  50.18 &
  \underline{ 49.32} &
  52.26 &
  50.63 &
  46.74 &
  49.76 &
  52.35 &
  44.96 \\ \hline
instruct + pos (2) &
  12.36 &
  42.14 &
  44.51 &
  52.37 &
  48.99 &
  \underline{ 53.99} &
  53.46 &
  52.73 &
  50.34 &
  54.79 &
  46.36 \\ \hline
instruct + pos (2) + neg (2) &
  14.02 &
  42.33 &
  43.57 &
  51.78 &
  48.57 &
  53.53 &
  \underline{ 54.28} &
  50.19 &
  49.56 &
  53.76 &
  45.94 \\ \hline
instruct + pos (2) + neg (2) + expl. &
  15.42 &
  41.98 &
  43.75 &
  50.72 &
  47.55 &
  51.88 &
  52.46 &
  \underline{ 52.62} &
  48.62 &
  52.24 &
  44.32 \\ \hline
pos (4) &
  10.98 &
  23.93 &
  45.58 &
  49.84 &
  48.99 &
  51.68 &
  49.55 &
  47.50 &
  \underline{ 49.75} &
  51.34 &
  44.45 \\ \hline
instruct + pos (4) &
  11.02 &
  42.39 &
  44.26 &
  51.85 &
  48.66 &
  53.68 &
  53.42 &
  50.61 &
  50.45 &
  \underline{ 53.54} &
  46.33 \\ \hline
\end{tabular}%
}
\caption{Performance when the model is trained with one type of instruction encoding and tested with another type of instruction encoding. Diagonal cells (underlined) represent model's performance when trained and tested with the same instruction encoding. Each encoding is one combination of the natural instruction elements in Fig \ref{fig:schema}. \textbf{Instruct} represents the task definition; \textbf{pos (k)} represents $k$ positive examples; \textbf{neg (k)} represents $k$ negative examples; \textbf{expl.} represents explanation.}
\label{tab:transferring_across_encodings}
\end{table*}
